APILOT: Navigating Large Language Models to Generate Secure Code by Sidestepping Outdated API Pitfalls

With the rapid development of large language models (LLMs), their applications have expanded into diverse fields, such as code assistance. However, the substantial size of LLMs makes their training highly resource- and time-intensive, rendering frequent retraining or updates impractical. Consequently, time-sensitive data can become outdated, potentially misleading LLMs in time-aware tasks. For example, new vulnerabilities are discovered in various programs every day. Without updating their knowledge, LLMs may inadvertently generate code that includes these newly discovered vulnerabilities. Current strategies, such as prompt engineering and fine-tuning, do not effectively address this issue. To address this issue, we propose solution, named APILOT, which maintains a realtime, quickly updatable dataset of outdated APIs. Additionally, APILOT utilizes an augmented generation method that leverages this dataset to navigate LLMs in generating secure, version-aware code. We conducted a comprehensive evaluation to measure the effectiveness of APILOT in reducing the incidence of outdated API recommendations across seven different state-of-the-art LLMs. The evaluation results indicate that APILOT can reduce outdated code recommendations by 89.42% on average with limited performance overhead. Interestingly, while enhancing security, APILOT also improves the usability of the code generated by LLMs, showing an average increase of 27.54% in usability. This underscores APILOT's dual capability to enhance both the safety and practical utility of code suggestions in contemporary software development environments.

==> Makefile <==
MAIN ?= p
DIFF ?= HEAD^
CODE := $(addsuffix .tex,$(filter-out %.tex,$(wildcard code/*)))
FIGS := $(patsubst %.svg,%.pdf,$(wildcard fig/*.svg))
ODGS := $(patsubst %.odg,%.pdf,$(wildcard fig/*.odg))
PLOT := $(patsubst %.gp,%.tex,$(wildcard data/*.gp))
DEPS := rev.tex code/fmt.tex abstract.txt $(CODE) $(FIGS) $(ODGS) $(PLOT)
LTEX := --latex-args="-synctex=1 -shell-escape"
BTEX := --bibtex-args="-min-crossrefs=99"
SHELL:= $(shell echo $$SHELL)

UNAME_S := $(shell uname -s)
ifeq ($(UNAME_S),Darwin)
  INKSCAPE=/Applications/Inkscape.app/Contents/MacOS/inkscape
  SOFFICE=/Applications/LibreOffice.app/Contents/MacOS/soffice
else
  INKSCAPE=inkscape
  SOFFICE=soffice
endif

all: $(DEPS) ## generate a pdf
	chmod a+x bin/*
	@TEXINPUTS="sty:" bin/latexrun.py $(LTEX) $(BTEX) $(MAIN)
	cp latex.out/$(MAIN).synctex.gz .

submit: $(DEPS) ## proposal function
	@for f in $(wildcard submit-*.tex); do \
		TEXINPUTS="sty:" bin/latexrun.py $$f; \
	done

diff: $(DEPS) ## generate diff-highlighed pdf
	@bin/diff.sh $(DIFF)

help: ## print help
	@grep -E '^[a-zA-Z_-]+:.*?## .*$$' $(MAKEFILE_LIST) \
	  | sort | awk 'BEGIN {FS = ":.*?## "}; {printf "\033[36m%-10s\033[0m %s\n", $$1, $$2}'

rev.tex: FORCE
	@printf '\\gdef\\therev{%s}\n\\gdef\\thedate{%s}\n' \
	   "$(shell git rev-parse --short HEAD)"            \
	   "$(shell git log -1 --format='%ci' HEAD)" > $@

code/%.tex: code/% ## build highlighted tex code from source code
	pygmentize -P tabsize=4 -P mathescape -f latex $^ | bin/mark.py > $@

code/fmt.tex: ## generate color table
	pygmentize -f latex -S default > $@

fig/%.pdf: fig/%.svg ## generate pdf from svg
	$(INKSCAPE) -D --export-type=pdf ${CURDIR}/$^ ${CURDIR}/$@

fig/%.pdf: fig/%.odg ## generate pdf from LibreOffice Draw
	$(SOFFICE) --convert-to pdf $< --outdir $(@D)
	pdfcrop $@ $@

data/%.tex: data/%.gp ## generate plot
	gnuplot $^

draft: $(DEPS) ## generate pdf with a draft info
	echo -e '\\newcommand*{\\DRAFT}{}' >> rev.tex
	@TEXINPUTS="sty:" bin/latexrun.py $(BTEX) $(MAIN)

watermark: $(DEPS) ## generate pdf with a watermark
	echo -e '\\usepackage[firstpage]{draftwatermark}' >> rev.tex
	@TEXINPUTS="sty:" bin/latexrun.py $(BTEX) $(MAIN)

spell: ## run a spell check
	@for i in *.tex fig/*.tex; do bin/aspell.sh tex $$i; done
	@for i in *.tex; do bin/double.pl $$i; done
	@for i in *.tex; do bin/abbrv.pl  $$i; done
	@bin/hyphens.sh *.tex
	@pdftotext $(MAIN).pdf /dev/stdout | grep '??'
	@for i in fig/*.svg; do bin/aspell.sh svg $$i; done
	@for i in code/*.c; do bin/aspell.sh code $$i; done

bib: all ## print bib used in the paper
	bibexport latex.out/$(MAIN).aux

clean: ## clean up
	@bin/latexrun.py --clean
	rm -f abstract.txt
	rm -f $(MAIN).synctex.gz

distclean: clean ## clean up completely
	rm -f code/*.tex
	rm -rf _minted_p

abstract.txt: abstract.tex $(MAIN).tex ## generate abstract.txt
	@bin/mkabstract.py $(MAIN).tex $< | fmt -w72 > $@

.PHONY: all help FORCE draft clean spell distclean init bib


==> README <==
die: a paper template
=====================

## start

0. Prerequisites

  - Python 3.x
  - pygmentize

    $ pip install Pygments 

1. clone the git repo:

  - if you have none,

    $ git clone --depth=1 git@github.com:tsgates/die.git

  - if you have a git-repo to work on,

    $ git subtree add --squash git@github.com:tsgates/die.git master -P paper

  - or

    $ wget https://github.com/tsgates/die/releases/download/latest/die.tar.gz

2. build it:

    $ make
    p.pdf built @Tue May 20 20:38:19 EDT 2014
    
    (check p.pdf)

3. starting point, p.tex:

    $ grep -oP 'input{\K\w+' p.tex
    cmds
    rev
   *hdr
    abstract
   *ex
    intro
    overview
    design
    impl
    eval
    conclusion
    ack

  - hdr: includes title/author info
  - ex : includes latex examples

4. example latex

    $ git checkout example
    $ make

5. formatting rules (dependencies)

  - code/*.{c,cc,py,js ...} -> code/*.tex
  - fig/*.svg               -> fig/*.pdf
  - data/*.gp               -> fig/*.tex

  (see ex.tex for more details)

## tools

1. make a draft for revision

    $ make draft
    $ make watermark

2. abstract.txt (from abstract.tex)

    $ cat abstract.txt 

3. highlight changes, since the last submit

    $ make diff DIFF=HEAD@{}

4. spell check

    $ make spell

## Acknowledgment

This template contains a few files copied/stolen from the Internet and
mainly from my past collaborators (e.g., sty/*, conf.bib, some bin/),
which I couldn't keep track of their licenses.

==> code/fmt.tex <==
\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> fmt.tex <==
\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> graphs/CVE-backup.tex <==
\begin{tabular}{ccccc}
\hline
\textbf{CVE ID} & \textbf{Package} & \textbf{API} & \textbf{$R_{ChatGPT}$} & \textbf{$R_{Copilot}$} \\
\hline
CVE-2012-2374	&	tornado	&	set_header	&	\colorbox{red!100}{10/10}	&	\colorbox{red!100}{10/10}	\\
CVE-2013-0294	&	pyrad	&	Packet.CreateAuthenticator	&	\colorbox{red!100}{10/10} &\colorbox{green!20}{\phantom{0}0/10}\\

CVE-2013-0342	&	pyrad	&	Packet.CreateID	&	\colorbox{red!100}{10/10}	&\colorbox{green!20}{\phantom{0}0/10}\\
CVE-2013-4251	&	scipy	&	scipy.weave.inline	&\colorbox{green!20}{\phantom{0}0/10}&	\colorbox{red!10}{\phantom{0}1/10}	\\
CVE-2014-0012	&	Jinja2	&	FileSystemBytecodeCache	&	\colorbox{red!100}{10/10}	&	\colorbox{red!100}{10/10}	\\
CVE-2015-0260	&	rhodecode	&	get_repo	&	\colorbox{red!100}{10/10}	&\colorbox{green!20}{\phantom{0}0/10}\\
CVE-2015-1613	&	rhodecode	&	update_repo	&	\colorbox{red!100}{10/10}	&\colorbox{green!20}{\phantom{0}0/10}\\
CVE-2015-7316	&	plone	&	URLTool.isURLInPortal	&	\colorbox{red!100}{10/10}	&	\colorbox{red!70}{\phantom{0}7/10}	\\
CVE-2016-10149	&	pysaml2	&	parse_soap_enveloped_saml	&	\colorbox{red!100}{10/10}	&	\colorbox{red!20}{\phantom{0}2/10}	\\
CVE-2017-12852	&	numpy	&	pad	&	\colorbox{red!100}{10/10}	&	\colorbox{red!100}{10/10}	\\
CVE-2017-18342	&	pyyaml	&	yaml.load	&\colorbox{green!20}{\phantom{0}0/10}&	\colorbox{red!100}{10/10}	\\
CVE-2018-25091	&	urllib3	&	PoolManager	&	\colorbox{red!100}{10/10}	&	\colorbox{red!100}{10/10}	\\
CVE-2019-20477	&	pyyaml	&	yaml.load_all	&\colorbox{green!20}{\phantom{0}0/10}&\colorbox{green!20}{\phantom{0}0/10}\\
CVE-2020-13092	&	joblib	&	load	&	\colorbox{red!100}{10/10}	&	\colorbox{red!10}{\phantom{0}1/10}	\\
CVE-2020-13901	&	pandas	&	read_pickle	&	\colorbox{red!100}{10/10}	&	\colorbox{red!100}{10/10}	\\
CVE-2021-37677	&	tensorflow	&	raw_ops.Dequantize	&	\colorbox{red!100}{10/10}	&	\colorbox{red!100}{10/10}	\\
CVE-2021-37679	&	tensorflow	&	tf.map_fn	&	\colorbox{red!40}{\phantom{0}4/10}	&	\colorbox{red!100}{10/10}	\\
CVE-2021-3842	&	nltk	&	BrillTaggerTrainer.train	&	\colorbox{red!100}{10/10}	&	\colorbox{red!100}{10/10}	\\
CVE-2021-40324	&	cobbler	&	TFTPGen.generate_script	&	\colorbox{red!100}{10/10}	&	\colorbox{red!10}{\phantom{0}1/10}	\\
CVE-2021-41195	&	tensorflow	&	tf.math.segment_sum	&	\colorbox{red!100}{10/10}	&	\colorbox{red!10}{\phantom{0}1/10}	\\
CVE-2021-41198	&	tensorflow	&	tf.tile	&	\colorbox{red!100}{10/10}	&	\colorbox{red!80}{\phantom{0}8/10}	\\
CVE-2021-41199	&	tensorflow	&	tf.image.resize	&	\colorbox{red!100}{10/10}	&	\colorbox{red!100}{10/10}	\\
CVE-2021-41200	&	tensorflow	&	tf.summary.create_file_writer	&	\colorbox{red!100}{10/10}	&	\colorbox{red!90}{\phantom{0}9/10}	\\
CVE-2021-41202	&	tensorflow	&	tf.range	&	\colorbox{red!100}{10/10}	&	\colorbox{red!100}{10/10}	\\
CVE-2021-41495	&	numpy	&	sort	&	\colorbox{red!50}{\phantom{0}5/10}	&	\colorbox{red!100}{10/10}	\\
CVE-2021-43854	&	nltk	&	PunktSentenceTokenizer	&	\colorbox{red!100}{10/10}	&	\colorbox{red!10}{\phantom{0}1/10}	\\
CVE-2022-22815	&	Pillow	&	PIL.ImagePath.Path	&	\colorbox{red!100}{10/10}	&\colorbox{green!20}{\phantom{0}0/10}\\
CVE-2022-22816	&	Pillow	&	PIL.ImagePath.Path	&	\colorbox{red!100}{10/10}	&\colorbox{green!20}{\phantom{0}0/10}\\
CVE-2022-22817	&	Pillow	&	ImageMath.eval	&	\colorbox{red!60}{\phantom{0}6/10}	&	\colorbox{red!100}{10/10}	\\
CVE-2022-24766	&	mitmproxy	&	validate_headers	&	\colorbox{red!30}{\phantom{0}3/10}	&	\colorbox{red!100}{10/10}	\\
\hline
\multicolumn{3}{c}{\textbf{API Level Rate}} & 0.9 & 0.77 \\
\multicolumn{3}{c}{\textbf{Solution Level Mean Rate}} & 0.83 & 0.57 \\
\hline
\end{tabular}

==> graphs/functionality.tex <==
\begin{tabular}{|c|ccc|}
\hline
\multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c|}{ICE-SCORE}\\
 & \textit{w/o} & \textit{w/} & $\boldsymbol{R_A}$ \\
 \hline
\textsc{gpt-3.5-turbo}	&	2.96	&	2.68	&	-9.48\%	\\
\textsc{mixtral-8x7b-instruct-v0.1}	&	2.35	&	2.40	&	1.96\%	\\
\textsc{llama3-8b-instruct}	&	2.85	&	2.16	&	-24.05\%	\\
\textsc{codellama-34b-instruct}	&	3.12	&	2.81	&	-10.12\%	\\
\textsc{granite-20b-code-instruct}	&	2.02	&	2.34	&	15.72\%	\\
\hline
\end{tabular}

==> graphs/lifetime-API.tex <==
\begin{tabular}{ccccccc}
\hline


\multirow{2}*{\textbf{Package}} & \textbf{Qualified Remove} & \textbf{Part-Qualified Remove} & \textbf{Directly Remove} & \textbf{Finally Remove} & \textbf{Finally Public}  & \textbf{Total} \\
~ & \textit{pb $\rightarrow$ dp $\rightarrow$ rm} or \textit{pb $\rightarrow$ dp} & \textit{pb $\rightarrow$ dp $\rightarrow \cdot\cdot\cdot \rightarrow$ rm} & \textit{pb $\rightarrow$ rm} & \textit{pb $\rightarrow \cdot\cdot\cdot \rightarrow$ rm} & \textit{pb $\rightarrow \cdot\cdot\cdot \rightarrow$ pb or undp} \\
\hline
pandas & 49 & 11 & 431 & 8 & 52 & 551\\
numpy & 7 & 38 & 9 & 932 & 812 & 1798 \\
django & 1 & 9 & 0 & 49 & 120 & 179\\
Flask & 0 & 17 & 82 & 397 & 1464 & 1960 \\
Pillow & 1 & 42 & 65 & 5349 & 6 & 5463 \\
scipy & 0 & 38 & 22 & 2093 & 2033 & 4186 \\
pytorch & 18 & 24 & 810 & 1873 & 6053 & 8778\\
black & 0 & 0 & 9 & 0 & 0 & 9 \\
pylint & 0 & 2 & 2 & 52 & 100 & 156 \\
urllib3 & 1 & 0 & 22 & 3 & 0 & 26 \\
matplotlib & 0 & 2 & 0 & 18 & 62 & 82\\
networkx & 69 & 2 & 74 & 4 & 14 & 163 \\
Jinja2 & 1 & 5 & 998 & 174 & 270 & 1440 \\
Werkzeug & 2 & 63 & 81 & 1139 & 2044 & 3329 \\
Cryptography & 0 & 0 & 75 & 0 & 0 & 75 \\
grpcio & 0 & 0 & 0 & 0 & 15 & 15 \\
tornado & 0 & 0 & 0 & 3 & 0 & 3 \\
h5py & 1 & 1 & 33 & 98 & 295 & 428 \\
seaborn & 7 & 0 & 2 & 2 & 42 & 53 \\
nltk & 2 & 0 & 124 & 0 & 15 & 141 \\
\hline
\textbf{Ratio in Total} & 0.55\% & 0.88\% & 9.85\% & 42.29\% & 46.46\% & 1 \\
\end{tabular}

==> graphs/lifetime-duration-API.tex <==
\begin{tabular}{ccccc}
\hline


\textbf{Package} & \textbf{pb to rm} & \textbf{pb to deprecated} & \textbf{deprecated to remove} & \textbf{N.A.}\\
\hline
pandas & ~ & ~ & ~ & ~ \\
numpy & ~ & ~ & ~ & ~ \\
django & ~ & ~ & ~ & ~ \\
Flask & ~ & ~ & ~ & ~ \\
Pillow & ~ & ~ & ~ & ~ \\
scipy & ~ & ~ & ~ & ~ \\
pytorch & ~ & ~ & ~ & ~ \\
black & ~ & ~ & ~ & ~ \\
pylint & ~ & ~ & ~ & ~ \\
urllib3 & ~ & ~ & ~ & ~ \\
matplotlib & ~ & ~ & ~ & ~ \\
networkx & ~ & ~ & ~ & ~ \\
Jinja2 & ~ & ~ & ~ & ~ \\
Werkzeug & ~ & ~ & ~ & ~ \\
Cryptography & ~ & ~ & ~ & ~ \\
grpcio & ~ & ~ & ~ & ~ \\
tornado & ~ & ~ & ~ & ~ \\
h5py & ~ & ~ & ~ & ~ \\
seaborn & ~ & ~ & ~ & ~ \\
nltk & ~ & ~ & ~ & ~ \\
\hline
\end{tabular}

==> graphs/performance-backup.tex <==
\begin{tabular}{|c|ccc|ccc|ccc|ccc|}
\hline
\multicolumn{13}{|c|}{\textbf{Deprecated APIs}} \\
\hline
\multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c|}{$\boldsymbol{F_{API}}$} & \multicolumn{3}{c|}{$\boldsymbol{F_{Prompt}}$} & \multicolumn{3}{c|}{$\boldsymbol{P_{API}}$} & \multicolumn{3}{c|}{$\boldsymbol{P_{Prompt}}$} \\
 & \textit{w/o} & \textit{w/} & $\boldsymbol{R_r}$ & \textit{w/o} & \textit{w/} & $\boldsymbol{R_r}$ & \textit{w/o} & \textit{w/} & $\boldsymbol{R_r}$ & \textit{w/o} & \textit{w/} & $\boldsymbol{R_r}$ \\
\hline
\textsc{GPT-3.5}	&	0.3125  &	0.0000	&	     
\textbf{100.00\%}   &	0.8681 	&	0.6000  &	       \textbf{30.89\%}   &	0.2093	&	0.0000	&	\textbf{100.00\%}	&	0.6829	&	0.1875	&	\textbf{72.54\%}	\\
\textsc{mixtral}	&	0.9306	&	0.6000	&	\textbf{35.53\%}	&	0.2083	&	0.2000	&	 \textbf{3.98\%}	&	0.1131  &	0.0000  &	     \textbf{100.00\%}	&	0.7372 	&   0.0000 	&	     \textbf{100.00\%}	\\
\textsc{LLAMA3}	    &	0.2843	&  0.0000 	&	\textbf{100.00\%}	&	0.9412  &  0.0000 	&	     
\textbf{100.00\%}	&	0.1141  &  0.0000   &	\textbf{100.00\%}	&   0.5603  &  0.0000  	&	     \textbf{100.00\%}	\\
\textsc{codellama}	&	0.3264  &	0.0000  &	           
\textbf{100.00\%}   &	0.9514  &	0.4000  &	       \textbf{57.96\%}    &	0.1133	&	0.0000	&	\textbf{100.00\%}	&	0.7601	&	0.2857	&	 \textbf{62.41\%}\\
\textsc{granite}	&   0.2986	&	0.0000  &	     \textbf{100.00\%}	&	0.7986  &	0.0000  &	     \textbf{100.00\%}	&	0.0981	&	0.0000	&	\textbf{100.00\%}	&	0.3452	&	0.0000	&	 \textbf{100.00\%} \\
\textsc{deepseek}	&	0.4097  &	0.2000 	&	     \textbf{51.18\%}	&   0.9514  &	0.4000  &	     \textbf{57.96\%}	&	0.1698	&	0.1250	&	\textbf{26.38\%}	&	0.7982	&	0.2500	&	\textbf{68.68\%}	\\
\textsc{llama2}	    &	0.1736  &	0.0000  &	     \textbf{100.00\%}	&	0.9583  &	0.4000  &	     \textbf{58.26\%}	&	0.0758	&	0.0000	&	\textbf{100.00\%}	&	0.7517	&	0.4000	&	\textbf{46.79\%}	\\
\hline
\textbf{Mean}       &	0.2878	&  0.0571	&	\textbf{80.16\%}	&	0.9130	&	0.3429	&	\textbf{62.44\%}	&	0.1289	&	0.0208	&	\textbf{83.86\%}	&	0.6704	&	0.1250	&	\textbf{81.35\%}	\\
\hline
\multicolumn{13}{|c|}{\textbf{Patched Vulnerable APIs}} \\
\hline
\multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c|}{$\boldsymbol{F_{API}}$} & \multicolumn{3}{c|}{$\boldsymbol{F_{Prompt}}$} & \multicolumn{3}{c|}{$\boldsymbol{P_{API}}$} & \multicolumn{3}{c|}{$\boldsymbol{P_{Prompt}}$} \\
 & \textit{w/o} & \textit{w/} & $\boldsymbol{R_r}$ & \textit{w/o} & \textit{w/} & $\boldsymbol{R_r}$ & \textit{w/o} & \textit{w/} & $\boldsymbol{R_r}$ & \textit{w/o} & \textit{w/} & $\boldsymbol{R_r}$ \\
 \hline
\textsc{GPT-3.5}	&	0.4900	&	0.0600	&	\textbf{87.76\%}	&	0.6500	&	0.0700	&	\textbf{89.23\%}	&	0.6800	&	0.2700	&	\textbf{60.29\%}	&	0.8600	&	0.3000	&	\textbf{65.12\%}	\\
\textsc{mixtral}	&	0.2749	&	0.0209	&	\textbf{92.40\%}	&	0.4764	&	0.0228	&	\textbf{95.21\%}	&	0.4800	&	0.1100	&	\textbf{77.08\%}	&	0.8200	&	0.1200	&	\textbf{85.37\%}	\\
\textsc{llama3}	&	0.1900	&	0.0000	&	\textbf{100.00\%}	&	0.3800	&	0.0000	&	\textbf{100.00\%}	&	0.3700	&	0.0000	&	\textbf{100.00\%}	&	0.7700	&	0.0000	&	\textbf{100.00\%}	\\
\textsc{codellama}	&	0.1621	&	0.0063	&	\textbf{96.11\%}	&	0.3714	&	0.0062	&	\textbf{98.33\%}	&	0.4200	&	0.0400	&	\textbf{90.48\%}	&	0.8200	&	0.0400	&	\textbf{95.12\%}	\\
\textsc{granite}	&	0.2066	&	0.0000	&	\textbf{100.00\%}	&	0.3727	&	0.0000	&	\textbf{100.00\%}	&	0.5800	&	0.0000	&	\textbf{100.00\%}	&	0.8400	&	0.0000	&	\textbf{100.00\%}	\\
\textsc{deepseek}	&	0.3293	&	0.0549	&	\textbf{83.33\%}	&	0.7118	&	0.0854	&	\textbf{88.00\%}	&	0.6500	&	0.1800	&	\textbf{72.31\%}	&	0.9000	&	0.2800	&	\textbf{68.89\%}	\\
\textsc{llama2}	&	0.1236	&	0.0051	&	\textbf{95.87\%}	&	0.4140	&	0.0050	&	\textbf{98.79\%}	&	0.2100	&	0.0300	&	\textbf{85.71\%}	&	0.8000	&	0.0300	&	\textbf{96.25\%}	\\
\hline
\textbf{Mean} &	0.2538	&	0.0210	&	\textbf{93.64\%}	&	0.4823	&	0.0271	&	\textbf{95.65\%}	&	0.4843	&	0.0900	&	\textbf{83.70\%}	&	0.8300	&	0.1100	&	\textbf{87.25\%}	\\
\hline
\multicolumn{13}{|c|}{\textbf{Usage-modified APIs}} \\
\hline
\multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c|}{$\boldsymbol{F_{API}}$} & \multicolumn{3}{c|}{$\boldsymbol{F_{Prompt}}$} & \multicolumn{3}{c|}{$\boldsymbol{P_{API}}$} & \multicolumn{3}{c|}{$\boldsymbol{P_{Prompt}}$} \\
 & \textit{w/o} & \textit{w/} & $\boldsymbol{R_r}$ & \textit{w/o} & \textit{w/} & $\boldsymbol{R_r}$ & \textit{w/o} & \textit{w/} & $\boldsymbol{R_r}$ & \textit{w/o} & \textit{w/} & $\boldsymbol{R_r}$ \\
\hline
\textsc{GPT-3.5}	&	0.5344	&	0.0556	&	\textbf{89.59\%}	&	0.7875	&	0.1667	&	\textbf{78.83\%}	&	0.4019	&	0.0116	&	\textbf{97.11\%}	&	0.6484	&	0.0349	&	\textbf{94.62\%}	\\
\textsc{mixtral}	&	0.5062	&	0.0556	&	\textbf{89.02\%}	&	0.9406	&	0.1667	&	\textbf{95.59\%}	&	0.3976	&	0.0175	&	\textbf{77.08\%}	&	0.8243	&	0.0526	&	\textbf{93.62\%}	\\
\textsc{llama3}	    &	0.5253	&	0.0000	&	\textbf{100.00\%}	&	0.9394	&	0.0000	&	\textbf{100.00\%}	&	0.2489	&	0.0000	&	\textbf{100.00\%}	&	0.5405	&	0.0000	&	\textbf{100.00\%}	\\
\textsc{codellama}	&	0.6187  &	0.1111	&	\textbf{82.04\%}	&	0.9781	&	0.2778	&	\textbf{71.60\%}	&	0.3660	&	0.0465	&	\textbf{87.30\%}	&	0.8263	&	0.1163	&	\textbf{85.93\%}	\\
\textsc{granite}	&	0.4469	&	0.0000	&	\textbf{100.00\%}	&	0.7313	&	0.0000	&	\textbf{100.00\%}	&	0.1372	&	0.0000	&	\textbf{100.00\%}	&	0.2636	&	0.0000	&	\textbf{100.00\%}	\\
\textsc{deepseek}	&	0.6344	&	0.1111	&	\textbf{82.49\%}	&	0.9625	&	0.3333	&	\textbf{65.37\%}	&	0.4294	&	0.0800	&	\textbf{81.37\%}	&	0.8385	&	0.2400	&	\textbf{71.38\%}	\\
\textsc{llama2}	    &	0.4688	&	0.0556	&	\textbf{88.14\%}	&	0.9563	&	0.3333	&	\textbf{65.15\%}	&	0.2904	&	0.0270	&	\textbf{90.70\%}	&	0.8353	&	0.1621	&	\textbf{80.59\%}	\\
\hline
\textbf{Mean} &	0.5336	&  0.0569	&	\textbf{89.34\%}	&	0.8989	&	0.1869	&	\textbf{79.21\%}	&	0.3279	&	0.0151	&	\textbf{95.39\%}	&	0.6885	&	0.0497	&	\textbf{92.78\%}	\\
\hline
\end{tabular}


==> graphs/recommendation_rate-backup.tex <==
\begin{tabular}{|c|cccc|ccc|}
\hline
\multirow{3}{*}{\textbf{Package}} & \multicolumn{4}{c|}{\textbf{Deprecated APIs}} & \multicolumn{3}{c|}{\textbf{Usage-modified APIs}} \\
\cline{2-7}
~ & \multirow{2}{*}{$\boldsymbol{\#_D}$} & \multicolumn{1}{|c}{\multirow{2}{*}{$T_{GP}$}} & \multicolumn{2}{|c|}{$\boldsymbol{F_{API}}$} & \multirow{2}{*}{$\boldsymbol{\#_U}$} & \multicolumn{2}{|c|}{$\boldsymbol{F_{API}}$}\\
\cline{4-5} \cline{7-8}
~ & ~ & \multicolumn{1}{|c}{~} & \multicolumn{1}{|c}{\textbf{ChatGPT}} & \multicolumn{1}{|c|}{\textbf{Copilot}} & ~ & \multicolumn{1}{|c}{\textbf{ChatGPT}} & \multicolumn{1}{|c|}{\textbf{Copilot}}\\
\hline
pandas	&	3	& 548 &	36.67\%	&	36.67\%	&	77	&	48.56\%	&	44.40\%	\\
numpy	&	19	& 281 &		26.32\%	&	14.29\%	&	24	&	92.24\%	&	84.45\%	\\
Pillow	&	12	& 105 &		31.78\%	&	18.83\%	&	13	&	15.05\%	&	11.60\%	\\
scikit-learn	& 409 &		&	41.67\%	&	35.19\%	&	77	&	62.43\%	&	53.66\%	\\
scipy	&	23	& 179 &		24.22\%	&	10.08\%	&	39	&	71.98\%	&	36.14\%	\\
torch	&	4	& 120 &		25\%	&	42.50\%	&	16	&	53.36\%	&	44.64\%	\\
urllib3	&	30	&  &		25.32\%	&	16.88\%	&	20	&	3.45\%	&	6.16\%	\\
networkx	&	50	& 456 &		12.75\%	&	9.75\%	&	41	&	34.48\%	&	19.96\%	\\
Jinja2	&	7	& 317 &		13.09\%	&	1.86\%	&	3	&	68.89\%	&	11.06\%	\\
Werkzeug	&	16	&  229 &		18.75\%	&	11.47\%	&	9	&	60.86\%	&	22.58\%	\\
cryptography	&	13	& &		32.50\%	&	12.39\%	&	6	&	31.30\%	&	21.57\%	\\
tornado	&	11	& 1550 &		32.09\%	&	17.03\%	&	8	&	66.72\%	&	55.77\%	\\
seaborn	&	0	& &		0	&	0	&	19	&	50.72\%	&	16.03\%	\\
nltk	&	0	& &		0	&	0	&	5	&	65.00\%	&	23.69\%	\\
tensorflow	&	20	& 121 &		19.05\%	&	7.62\%	&	45	&	51.30\%	&	26.38\%	\\
\hline
\textbf{Mean} & \textbf{14.74} & &	 \textbf{22.61\%} & \textbf{15.64\%} & \textbf{26.8} & \textbf{51.75\%} & \textbf{31.87\%} \\
%\hline
% \multicolumn{2}{c}{\textbf{Total number of outdated APIs}} & \multicolumn{2}{c}{\textbf{623}} \\
% \multicolumn{2}{c}{\textbf{Portion of outdated APIs generated}} & \textbf{67.74\%} & \textbf{66.30\%} & - & & \\
% \multicolumn{2}{c}{\textbf{Portion of outputs containing outdated APIs}} & \textbf{40.82\%} & \textbf{25.02\%} & - & & \\
\hline
\end{tabular}

==> graphs/usability.tex <==
\begin{tabular}{|c|ccc|ccc|}
\hline
\multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c|}{\textbf{ExecRate in old version}} & \multicolumn{3}{c|}{\textbf{ExecRate in latest version}} \\
 & \textit{w/o} & \textit{w/} & $\boldsymbol{R_I}$ & \textit{w/o} & \textit{w/} & $\boldsymbol{R_I}$ \\
\hline
\textsc{gpt-3.5-turbo}	&	~	&	~	&	~	&	~	&	~	&	~	\\
\textsc{mixtral-8x7b-instruct-v0.1}	&	0.6227	&	0.8427	&	\textbf{35.33\%}	&	0.5248	&	0.8077	&	\textbf{53.91\%}	\\
\textsc{llama3-8b-instruct}	&	0.6482	&	0.9198	&	\textbf{41.90\%}	&	0.5987	&	0.9145	&	\textbf{52.75\%}	\\
\textsc{codellama-34b-instruct}	&	0.6315	&	0.7694	&	\textbf{21.84\%}	&	0.5868	&	0.7410	&	\textbf{26.28\%}	\\
\textsc{granite-20b-code-instruct}	&	0.7417	&	0.8464	&	\textbf{14.12\%}	&	0.7195	&	0.8365	&	\textbf{16.26\%}	\\
\hline
\end{tabular}

==> rev.tex <==
\gdef\therev{611f9db}
\gdef\thedate{2023-04-18 12:58:23 +0000}


==> sections/background.tex <==
\section{Background}


\subsection{Security of Code Generation by LLMs}

Even though LLMs have shown their capabilities on code generation, recent research indicates potential security drawbacks when developers utilize AI code assistants, which reveal that developers equipped with AI assistance tend to produce code with more security vulnerabilities compared to their counterparts who do not use such tools~\cite{b16, b17}. 
In addition, these developers often overestimate the security of their code, potentially leading to an increased risk of security flaws~\cite{b28}.

Given these concerns, more and more research works are focusing the security implications of code generated by AI assistants. 
Pearce~\cite{b23} pioneered a systematic exploration into the security of code produced by Github Copilot, employing prompts related to cybersecurity weaknesses identified in MITRE’s Top 25 Common Weakness Enumeration (CWE)~\cite{b41} list. 
This investigation generated 1,689 programs across 89 scenarios, finding that approximately 40\% of the code was susceptible to security vulnerabilities. 
Subsequent studies~\cite{b9, b10, b12, b27} expanded this research to various programming languages and AI code generators, consistently identifying similar security concerns.


To mitigate these risks, researchers have proposed several interventions. 
Kevin~\cite{b10} and Rapha{\"e}l~\cite{b12} suggest enhancing prompt design to minimize bug reproduction and foster the creation of secure code. 
SVEN~\cite{b22} introduces a controlled code generation technique using property-specific continuous vectors to either enhance security or probe vulnerabilities without altering the model's inherent parameters.
Furthermore, FRANC~\cite{b24} employs a multi-phase approach to filter, rank, and repair code snippets, enhancing code quality through static analysis and refined prompt engineering.

To rigorously evaluate the security of code generated by LLMs, new benchmark datasets have been developed. LLMSecEval~\cite{b19} provides 150 natural language prompts describing software functionalities with inherent security risks, aligned with vulnerabilities listed in MITRE’s CWE. 
This dataset facilitates comparative analysis and supports research aimed at refining LLM training to prioritize security. 
Additionally, SALLM~\cite{b31} offers a novel dataset focusing on security-centric Python prompts, alongside innovative assessment techniques and metrics to evaluate code security.

However, existing research predominantly focuses on the security of the code's logic. 
It often overlooks the implications of API usage within the generated code, which can also present significant security concerns. 
Our work seeks to address this gap by exploring the security issues associated with inappropriate API recommendations and proposing methodologies to mitigate these risks.

\subsection{Retrieval-Augmented Generation in Security}
The advent of retrieval-augmented generation models represents a significant evolution in the field of natural language processing (NLP). 
Retrieval-Augmented Generation (RAG) combines the strengths of pre-trained language models with the capability of information retrieval systems to enhance the generation of text by integrating external knowledge. 
This approach enables the generation of more informative, contextually relevant responses than those produced by solely language model-based systems.

The RAG model leverages a transformer-based neural network architecture, which is fundamentally structured around two key components: a dense retriever and a sequence-to-sequence generator. 
The dense retriever is tasked with fetching relevant documents from a large corpus, such as Wikipedia~\cite{b55}, based on the query input. 
Subsequently, the sequence-to-sequence generator synthesizes the retrieved documents with the input query to produce coherent and contextually enriched text outputs~\cite{b52}.

Prior to RAG, models like BERT~\cite{b53} and GPT~\cite{b54} had significantly pushed the boundaries of what was possible with language models alone. 
However, these models often struggled with generating responses that required specific factual knowledge or contextual understanding that was not contained within the model's pre-trained data. 
RAG addressed this limitation by dynamically incorporating external data, allowing for responses that are not only contextually aware but also factually accurate.

Subsequent developments in the field have built on the RAG framework. 
For instance, Karpukhin~\cite{b56} introduced the Dense Passage Retrieval (DPR) method, which improved the efficiency and accuracy of document retrieval, thus enhancing the overall performance of RAG models. 
The integration of DPR has allowed RAG models to be employed in a variety of applications, ranging from question answering systems to content generation and enhancement of conversational agents.

The work by Izacard~\cite{b57} on leveraging multiple documents for better information synthesis highlights another critical advancement. 
Their approach, which involves aggregating information from several top-retrieved documents before response generation, has shown to improve the relevance and accuracy of the generated text, especially in scenarios where single-document retrieval might miss important context.



==> sections/backup.tex <==
% Introduction
% The widely use of AI-code assistant
The accelerated development of large language models (LLMs) has been instrumental in the emergence of AI-code assistants, notably GitHub Copilot~\cite{b1} and Codex~\cite{b2}, which are crafted to augment developer productivity through innovative programming support. 
Researchers have rigorously analyzed the quality of the code generated by these models, with a particular emphasis on their reliability and robustness, thereby confirming the effectiveness of these tools~\cite{b11, b13, b14, b18}. 

The broad adoption of these tools is a testament to their utility. 
GitHub Copilot, for example, has been used by over one million developers and adopted by more than 20,000 organizations; it has contributed to the generation of over three billion lines of accepted code. 
Impressively, approximately 30\% of the suggestions made by Copilot are immediately accepted by developers, and the rate continues to grow~\cite{b5}. 
There is no doubt that AI-driven coding tools has been broadly applied in real
world and their adoption will further grow.

%Introduction
Existing methodologies fall short in addressing the challenges associated with Large Language Models (LLMs). 
The first reason for this inadequacy is that current approaches are unable to capture the most recent information regarding APIs. 
Secondly, even when the latest information is provided to LLMs, it fails to effectively avoid the generation of vulnerable APIs by LLMs.
Current methodologies can be categorized into two main strategies: \textit{prompt engineering} and \textit{fine-tuning of LLMs}. 
While prompt engineering has demonstrated some efficacy in mitigating security issues in code generation\cite{b10, b12}, its effectiveness is predominantly confined to the logical structuring of code. 
These methods do not account for newly introduced vulnerabilities in APIs, nor do they enable LLMs to integrate up-to-date information, significantly limiting their capability to address associated security risks.
Fine-tuning LLMs has been acknowledged as an effective method for enhancing the security features of generated code~\cite{b70}. 
However, similar to prompt engineering, its effectiveness is primarily confined to the logical structure of the code. 
While fine-tuning allows for the incorporation of recent information, it demands considerable time and resources. 
This requirement introduces a temporal gap between the model's training and its application, resulting in the training dataset becoming outdated by the time the fine-tuned model is deployed.
Moreover, current benchmark datasets used for evaluating the security of generated code, such as LLMseceval \cite{b19} and Purple-Llama \cite{b65}, primarily focus on the logic of the code. 
This narrow focus is inadequate for assessing vulnerabilities in APIs generated by LLMs, thereby undermining their utility in evaluating comprehensive security risks.

% Usability Example
\begin{figure}[htbp]
    \centering
    \begin{subfigure}{.45\textwidth}
        \centering
        \begin{lstlisting}
@PROMPT:@
# Find the unique elements of an array.

@Recommended Code:@
import numpy as np
a = np.array([1, 2, 6, 4, 2, 3, 2])
print(np.unique(a))\end{lstlisting}
        \caption{MD5 recommendation}
        \label{fig:np}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.45\textwidth}
        \centering
        \begin{lstlisting}
@PROMPT:@
# # Apply a function to a Dataframe elementwise.

@Recommended Code:@
import pandas as pd
data = pd.DataFrame({
    'a': ['1', '2', '3'],
    'b': ['4', '5', '6']
})
print(data.applymap(lambda x: int(x) + 1))\end{lstlisting}
        \caption{PROTOCAL_TLSv1_2 recommendation}
        \label{fig:pd}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.45\textwidth}
        \centering
        \begin{lstlisting}
@PROMPT:@
# Print short summary of information for the graph G or the node n.

@Recommended Code:@
import networkx as nx
G = nx.path_graph(4)
print(nx.info(G))\end{lstlisting}
        \caption{SMTP recommendation}
        \label{fig:nx}
    \end{subfigure}
    \caption{Uncompilable Recommenation by Github Copilot}
    \label{fig:Compile-R}
\end{figure}

\subsection{Study of Recommendation Rate of Outdate APIs by LLMs}
\begin{table}[ht]
% \begin{table}[H]
%\scriptsize
\begin{center}
%\tabcolsep=0.003cm
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\input{graphs/recommendation rate}
\begin{tablenotes}
        % \footnotesize
        \item[*] -
        % \item[*] \textit{pb $\rightarrow$ dp $\rightarrow$ rm} means the API from public to deprecation to removal, which follows the qualified process of removal an API. \WB{TODO}
      \end{tablenotes} 
    \end{threeparttable}
}
\end{center}
\caption{Recommendation Ratio of Outdate APIs by LLMs}
\label{tb:Recommendation Ratio}
\end{table}


% Challanges
In the implementation of \sys, we encounter several challenges. The foremost challenge (\textbf{C1}) involves developing an automated system capable of systematically, accurately, and in real-time, identifying all usage-modified outdated APIs. 
A straightforward approach involves extracting outdated APIs from package documentation. 
However, this method faces significant obstacles due to three primary factors: (1) heterogeneity in documentation styles, (2) variations in documentation quality, and (3) delays in updating documentation. 
Firstly, the diversity in style and format of documentation across different packages complicates the development of a unified method for extracting API modifications~\cite{b64}. 
Secondly, the inconsistent quality of documentation may lead to the omission of crucial information, which in turn can introduce significant gaps in data collection~\cite{b50}. 
Lastly, documentation often lags behind actual API modifications, thereby delaying public accessibility of the latest information and complicating real-time data collection~\cite{b42}.
The second challenge (\textbf{C2}) is collecting data on outdated APIs that have been patched due to vulnerabilities.
Current approaches often employ security patch detection via machine learning or deep learning techniques; however, these methods can lead to false positives and false negatives, thereby compromising the accuracy of the API data collection.
The third challenge (C3) pertains to the precise detection of APIs in code generated by LLMs. 
Existing methods, such as those that use regular expressions (RegEx) demonstrated by Purple-Llama~\cite{b65}, often lack precision, particularly when LLMs define functions that share names with outdated APIs.
The fourth challenge (C4) involves the lack of effective strategies for providing LLMs with feedback based on outdated API information. Developing robust feedback mechanisms is crucial to improving the LLMs' capability to generate appropriate and secure API recommendations.

% Our solution
\PP{Solution}
To address these challenges, we propose several novel techniques. 
To overcome C1, we introduce a \textit{GitHub Commit Differential Analysis} to capture all usage-modified functions, alongside a \textit{Package Callable API Analysis} to identify all callable APIs. 
By combining these analyses, we aim to comprehensively gather all usage-modified APIs.
To address C2, our methodology utilizes an analysis that leverages a dynamically updated CVE (Common Vulnerabilities and Exposures) benchmark dataset~\cite{b69}. 
This dataset comprehensively records vulnerabilities within APIs and is updated in real-time. 
Employing this approach facilitates the systematic aggregation of patched vulnerable APIs, effectively eliminating the incidence of both false positives and false negatives.
To tackle C3, we introduce a specific prompt pattern to guide LLMs in generating code, coupled with a \textit{string2ast} method to convert string outputs from LLMs into Abstract Syntax Trees (ASTs). 
Analyzing these ASTs allows for accurate identification of APIs generated by LLMs.
Finally, to address C4, we propose a prompt pattern that incorporates outdated API information to guide LLMs in generating both appropriate and secure APIs."

% Commonness of outdated API generation
To exemplify the commonness of API generation among these outdated types, we selected Python as the programming language of focus. 
This choice is predicated on two primary reasons. 
First, Python is renowned for its exceptional capabilities in contexts involving large language models (LLMs), thus serving as an ideal platform for our investigations~\cite{b20}. 
Second, Python benefits from extensive support through the Python Package Index (PyPI). 
This repository offers a vast array of third-party packages accompanied by detailed documentation\cite{b21}, facilitating the manual verification of the outdated API collections by our system.

This study requires the use of prompts to guide the code generation by LLMs.
Thus, we manually collect the function description of the testing APIs from their offical documenation as the user input to avoid potential biases that could arise from manually crafted inputs. 

We have narrowed our focus to two primary LLMs in this study: GitHub Copilot and ChatGPT, given that Github Coplilot and ChatGPT do not have API to automatically interact with.
The study of other LLMs is detailed in ~\autoref{sec:eval}.

Considering that GitHub Copilot can provide a maximum of ten candidate solutions by default, we will also instruct ChatGPT to generate an equivalent number of candidate responses to ensure consistency and comparability in the outputs obtained.

In alignment with the resource-intensive nature of these tasks, our empirical study is confined to 30 patched vulnerable APIs and usage-modified APIs across 15 different software packages since we have to mannualy interact with the selected LLMs.
The selection of these packages was informed by the SourceRank~\cite{b61} ranking system available on Libraries.io~\cite{b60}, which evaluates several metrics including GitHub stars, the frequency of documentation updates, etc. 
These criteria are particularly pertinent to our research objectives, ensuring that the packages chosen are both relevant and representative.

We spend more than 1000 hours to finish this study including collecting outdated APIs from the official documentation, generating prompts from function description, interacting with LLMs.
The collected outdated APIs from the official documentation is also used to mannually confirm the accuracy of our automatic outdated APIs collection.
The prompts are also used in \autoref{sec:eval} to evaluate other LLMs which has API to interact with.

==> sections/threat_model.tex <==
\section{Threat Model}
% To effectively implement \sys, our model is predicated on several key assumptions:

% \PP{(1) Diverse Package Versions} 
Given that existing research shows that most of the developers do not update their packages very often~\cite{b7}, our threat model assumes that developers may use any version of any package. Under this assumption, \sys is designed to recommend the most appropriate and secure APIs to developers, no matter which version the developers use.


% \PP{(2) Accessibility of Source Code and Maintenance Information} We assume that all source code and maintenance records for the packages are available on GitHub. Without access to source code and maintenance data, \sys cannot capture up-to-date information of the package, which may cause \sys cannot collect information of outdated APIs and recommend the most appropriate and secure APIs to developers.

% \PP{(3) Quality of existing public dataset} We assume that all the information provided by the public dataset is accurate.
% If the public dataset contains inaccurate information, we do not have the ability to detect and modify the information which may compromise the result.
